Ponimator: Unfolding Interactive Pose for Versatile Human-human Interaction Animation

Close-proximity human-human interactive poses convey rich contextual information about interaction dynamics. Given such poses, humans can intuitively infer the context and anticipate possible past and future dynamics, drawing on strong priors of human behavior. Inspired by this observation, we propose Ponimator, a simple framework anchored on proximal interactive poses for versatile interaction animation. Our training data consists of close-contact two-person poses and their surrounding temporal context from motion-capture interaction datasets. Leveraging interactive pose priors, Ponimator employs two conditional diffusion models: (1) a pose animator that uses the temporal prior to generate dynamic motion sequences from interactive poses, and (2) a pose generator that applies the spatial prior to synthesize interactive poses from a single pose, text, or both when interactive poses are unavailable. Collectively, Ponimator supports diverse tasks, including image-based interaction animation, reaction animation, and text-to-interaction synthesis, facilitating the transfer of interaction knowledge from high-quality mocap data to open-world scenarios. Empirical experiments across diverse datasets and applications demonstrate the universality of the pose prior and the effectiveness and robustness of our framework.

==> figs/fig_text2motion.tex <==
\begin{table*}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{0.2em} %
    \resizebox{0.85\linewidth}{!}{
        \begin{tabular}{ccccc}
        
        \vistm{vis_t2m/vis_interx}{G038T003A018R018}{05}{10}{15}{20}{25}

         \multicolumn{5}{c}{Input Text: One person goes to the other person's ear and whispers to him/her} \\

        \vistm{vis_t2m/vis_chi3d}{s02_Handshake_10}{05}{10}{15}{20}{25}

        \multicolumn{5}{c}{Input Text: hand shake} \\
         
    \end{tabular}
    }
\captionof{figure}{\textbf{Text-to-interaction motion synthesize}}

\label{fig:exp-t2m-results}
\end{table*}


==> preamble.tex <==
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}



==> supp_figs/fig_contact_diverse.tex <==
\begin{table*}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{0.2em} % Adjust horizontal padding
    \resizebox{\linewidth}{!}{
        \begin{tabular}{c|cccc}

        {Interactive Pose} & 
        \multicolumn{4}{c}{{Interaction Animation (left$\rightarrow$right: time steps)}} \\

    \includegraphics[width=0.2\linewidth]{rebuttal_src_figs/pair00_000040_1_10/00_crop.pdf} &
     \includegraphics[width=0.2\linewidth]{rebuttal_src_figs/pair00_000040_1_10/05_crop.pdf} &
      \fcolorbox{green}{white}{
      \includegraphics[width=0.2\linewidth]{rebuttal_src_figs/pair00_000040_1_10/10_crop.pdf}} & 
      \includegraphics[width=0.2\linewidth]{rebuttal_src_figs/pair00_000040_1_10/15_crop.pdf} &
      \includegraphics[width=0.2\linewidth]{rebuttal_src_figs/pair00_000040_1_10/19_crop.pdf} \\

    \includegraphics[width=0.2\linewidth]{rebuttal_src_figs/pair00_000040_1_20/05_crop.pdf} &
     \includegraphics[width=0.2\linewidth]{rebuttal_src_figs/pair00_000040_1_20/12_crop.pdf} &
      \includegraphics[width=0.2\linewidth]{rebuttal_src_figs/pair00_000040_1_20/15_crop.pdf} & 
      \fcolorbox{green}{white}{
      \includegraphics[width=0.2\linewidth]{rebuttal_src_figs/pair00_000040_1_20/20_crop.pdf}} &
      \includegraphics[width=0.2\linewidth]{rebuttal_src_figs/pair00_000040_1_20/23_crop.pdf} \\

    \end{tabular}
    }
\captionof{figure}{\textbf{Diverse interactive pose animation}. Given an interactive pose, we can synthesize different windows of past and future frames by adjusting the interactive time.}
\label{fig:exp-contact-diverse}
\end{table*}
